An Incremental Update Framework for Online Recommenders with Data-Driven Prior

Online recommenders have attained growing interest and created great revenue for businesses. Given numerous users and items, incremental update becomes a mainstream paradigm for learning large-scale models in industrial scenarios, where only newly arrived data within a sliding window is fed into the model, meeting the strict requirements of quick response. However, this strategy would be prone to overfitting to newly arrived data. When there exists a significant drift of data distribution, the long-term information would be discarded, which harms the recommendation performance. Conventional methods address this issue through native model-based continual learning methods, without analyzing the data characteristics for online recommenders. To address the aforementioned issue, we propose an incremental update framework for online recommenders with Data-Driven Prior (DDP), which is composed of Feature Prior (FP) and Model Prior (MP). The FP performs the click estimation for each specific value to enhance the stability of the training process. The MP incorporates previous model output into the current update while strictly following the Bayes rules, resulting in a theoretically provable prior for the robust update. In this way, both the FP and MP are well integrated into the unified framework, which is model-agnostic and can accommodate various advanced interaction models. Extensive experiments on two publicly available datasets as well as an industrial dataset demonstrate the superior performance of the proposed framework.

==> prelim.tex <==
\subsection{Preliminaries}
Assume each instance $(\mathcal{X},y)$ records a piece of impression, where $\mathcal{X}$ denotes features with $M$ fields, and $y \in \{0,1\}$ indicates whether the user clicks the item. After one-hot or multi-hot encoding for the features, each instance can be converted into $\mathbf{x}=[\mathbf{x}_1, ..., \mathbf{x}_M]$ where $\mathbf{x}_j $ denotes the encoding vector for the $j$-th field. The CTR-prediction model then learns a mapping $\hat{y} = f_{\theta} (\mathbf{x})$ to estimate the probability of user click. 
Previous models can be summarized with three parts: embedding module, interaction module and loss function. The embedding module convert encoding into embedding vector $\mathbf{e}=[\mathbf{e}_1, ..., \mathbf{e}_M]$, where $\mathbf{e}_j \in \mathbb{R}^d$ is obtained through the embedding matrix $\bm{E} \in \mathbb{R}^{N \times d}$. $N$ denotes the number of sparse feature values. The interaction module attempts to capture the complex relationships between features and to predict the probability of the user click through the sigmoid function, i.e., $\hat{y}= f_{\theta}(\mathbf{x}) = \sigma\left(\text{Interaction\_Module}(\mathbf{e})\right)$. $\theta$ denotes the set of parameters and $f(\cdot)$ summarizes all calculations.
% A great effort has been devoted to the design of the interaction models, such as DeepFM~\cite{guo2017deepfm} and DIN~\cite{zhou2018deep}, where the feature interactions are fully extracted to enhance the expressiveness. 
Finally, the model is optimized through the binary cross entropy loss $\mathcal{L(\mathcal{D}; \theta)}$.
% by maximum likelihood estimation.
% $\log p(\mathcal{D} | \theta)$.
%where $\mathcal{D}$ denotes training data.}


Considering the industrial scenarios under large scales, 
% the model update takes an extremely huge computational cost if all historical impressions are adopted. Thus, 
the incremental update becomes a popular framework, where the model is updated only with newly arrived data $\mathcal{D}_t$. $\mathcal{D}_t$ denotes the data collected from the period $t$, whereby a period can be a certain length of time (e.g., an hour, a day). $\mathcal{H}_{t}=\mathcal{D}_1 \cup \mathcal{D}_2 ,..., \cup \mathcal{D}_{t}$ denotes the historical training data up to the period $t$. Correspondingly, $\theta_{t-1}$ denotes model parameters updated in time $t-1$. The incremental update receives the newly arrived data $\mathcal{D}_{t}$ and previous model $\theta_{t-1}$, updating the model parameters, i.e., $\min \mathcal{L}(\mathcal{D}_{t}, \theta_{t-1}; \theta)$. It is obvious that the models are prone to overfitting to recent data when there is a drift of online data, and long-term user interest would be discarded under the loop of the incremental update. 
% Thus, to alleviate the problem, we propose a data-driven prior method for incremental update. 
